Versatile Locomotion Skills for Hexapod Robots

Hexapod robots are potentially suitable for carrying out tasks in cluttered environments since they are stable, compact, and light weight. They also have multi-joint legs and variable height bodies that make them good candidates for tasks such as stairs climbing and squeezing under objects in a typical home environment or an attic. Expanding on our previous work on joist climbing in attics, we train a legged hexapod equipped with a depth camera and visual inertial odometry (VIO) to perform three tasks: climbing stairs, avoiding obstacles, and squeezing under obstacles such as a table. Our policies are trained with simulation data only and can be deployed on lowcost hardware not requiring real-time joint state feedback. We train our model in a teacher-student model with 2 phases: In phase 1, we use reinforcement learning with access to privileged information such as height maps and joint feedback. In phase 2, we use supervised learning to distill the model into one with access to only onboard observations, consisting of egocentric depth images and robot pose captured by a tracking VIO camera. By manipulating available privileged information, constructing simulation terrains, and refining reward functions during phase 1 training, we are able to train the robots with skills that are robust in non-ideal physical environments. We demonstrate successful sim-to-real transfer and achieve high success rates across all three tasks in physical experiments.

==> figures/squeeze_graph.tex <==
\begin{figure}
    \vspace{0.2cm}
    \centering
    \frame{\includegraphics[width=88mm, clip]{images/squeeze height.png}}
    \caption{\textbf{Plot of the robot height vs. Number of rollout}: the height is sampled every rollout, and each rollout takes roughly 0.04 second to run on the physical robot.}
    \label{fig:s_g}
    \vspace{-0.5cm}
\end{figure}

==> figures/squezzing_table2.tex <==


\begin{table}[ht]
\centering
\begin{adjustbox}{width=0.5\textwidth,center}
\begin{tabular}{@{}lccc@{}}
\toprule
Method & 31.75 cm obstacle & 34.29 cm obstacle & 36.83 cm obstacle \\
\midrule
Perceptive (Ours) & \cmark & \cmark & \cmark \\
Blind & \xmark & \xmark & \cmark \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Robot's ability to walk through objects}. \cmark denotes success over 70\% and \xmark denotes success below 70\%}
\label{table:s2}
\end{table}


==> figures/stairs_design.tex <==
\begin{figure}
    \vspace{0.2cm}
    \centering
    \frame{\includegraphics[width=45mm]{images/stairs design.png}}
    \caption{\textbf{Physical design of a staircase}. Three key components of the stairs are defined as \textbf{width, depth, and height}. }
    \vspace{-0.7cm}
\label{fig:stairs}
\end{figure}

==> section-3-problem-statement.tex <==
% \section{Problem Statement}
% Given a hexapod robot (6 legs and 2 cameras), can the robot travel across a cluttered environment consisting of obstacles in the front, obstacles above, and stairs using reinforcement leaning and sim-to-real transfer? Can it choose relevant skills automatically by using large visual language models like ChatGPT-4V?

% We make the following assumptions: our hexapod robot is traveling straight in a light sufficient environment.

% At the beginning of experimentation, the hexapod robot is placed 50-100 centimeters away from the first obstacle


% Potential inputs to our lower-level skill models includes depth image from L515, pose estimation from T265; to our higher-level skill selection models are a processed gray scale image collected from T265 fisheye cameras and its corresponding depth images.



==> section-9-acknowledgements.tex <==
\section*{Acknowledgements}
\vspace{-0.1cm}
\relsize{-1}

